On the generalization of bayesian deep nets for multi-class classification

Generalization bounds which assess the difference between the true risk and the empirical risk have been studied extensively. However, to obtain bounds, current techniques use strict assumptions such as a uniformly bounded or a Lipschitz loss function. To avoid these assumptions, in this paper, we propose a new generalization bound for Bayesian deep nets by exploiting the contractivity of the Log-Sobolev inequalities. Using these inequalities adds an additional loss-gradient norm term to the generalization bound, which is intuitively a surrogate of the model complexity. Empirically, we analyze the affect of this loss-gradient norm term using different deep nets.

==> 4_bound_bu.tex <==
%!TEX root = main.tex
\section{Generalization Bound}

The challenge in deriving a generalization bound is bounding the log-partition function $\log \E_{w \sim p, S \sim D^m}  [ e^{ \lambda G_S(w) } ]$, where $G_S(w) = L_D(w) - L_S(w)$. In many cases of interest, the generalization gap $G_S(w)$ is uniformly bounded by a constant. In this case the log-partition function is bounded as well. Unfortunately, a uniform bound does not exist for the NLL loss $-(W_k x_k)_y + \log (\sum_{\hat y} e^{(W_k x_k)_{\hat y}} )$. For example, if the rows in $W_k$  consist of the vector $r x_k$ then the NLL loss increases with $r$, and is unbounded when $r \rightarrow \infty$.

%Our main theorem shows that following the work of \emph{Bayes-by-Backprop}~\citep{Blundell15} together with the Log-Sobolev inequality, allow us to bound the moment generating function of the risk using the squared norm of the gradients w.r.t the input. 
Our main theorem shows following the \emph{Herbst Argument} for the Log-Sobolev inequality when considering the log-partition function as the moment-generating function of the generalization, allows us bound it using the squared norm of the gradients w.r.t the input. Formally, 

\begin{theorem}
\label{thm:pac-bound-general-2}
Let $KL(q||p)$ be the KL-divergence between two probability density functions $p, q$. Let $M(\alpha) = \E_{(x,y) \sim D} e^{\alpha \ell(w, x, y)}$ be the moment generating function $\ell(w, x, y)$. Let $p$ be the probability density function of $N(0, \sigma_p^2 I)$, which is the prior distribution over the parameters $w$. With probability at least $1-\delta$ over the draw of the training set $S$ the following holds simultaneously for any posterior probability density function $q$ whose posterior distribution is $N(\mu_q, \operatorname{diag}(\sigma_q^2))$: 
\[
\E_{w \sim q} [G_S(w)] \le \frac{\log\E_{w \sim p} e^{C \frac{\lambda^2}{m} \E_{(x, y) \sim D}\big [ \| \nabla_{x} \ell(w, x, y) \| ^2 \int_0^1 \frac{ e^{\alpha \ell(w, x, y)} }{M(\alpha)}  d \alpha \big] +  KL(q || p) + \log(1/\delta)}}{\lambda}.\nonumber
\]
\end{theorem}

\adios{Can we summarize the proof in a few simple points?}
The proof consists of {\color{blue} XXX} steps which we briefly outline here:
\vspace{-\topsep}
\begin{enumerate}\setlength{\parskip}{0pt}\setlength\itemsep{0pt plus 1pt}
\item yoyoyo
\item whwhwhw
\end{enumerate}

Intuitively, the proposed bound is comprised of two terms: (i) the expressivity of the of the model over the prior distribution, which is dominated by the squared norm of the gradients w.r.t the input. (ii) satisfying the simplicity prior, which is the KL term.

\emph{Proof}. Denote $\mu$ as the prior distribution in the PAC-Bayesian setting. The moment-generating function of $f$ is defined as follows,
\begin{equation}
\label{eq:mgf}
M(\lambda) \stackrel{def}{=}  \E [e^{\lambda f}] = \int_{\R} e^{\lambda f(t)} d\mu(t).
\end{equation}

In the following, our goal is to bound $M(\lambda)$ (Eq.~\ref{eq:mgf}). In order to do so we first set $H(\lambda) = \frac{1}{\lambda}\log M(\lambda)$. Now, we can derive two properties:
\begin{enumerate}
\item 
\begin{equation}
\label{eq:lambda_derv}
\begin{split}
H'(\alpha) &= - \frac{\log M(\alpha)}{\alpha^2} + \frac{M'(\alpha)}{\alpha M(\alpha)} = \frac{ \alpha M'(\alpha) -  M(\alpha) \log M(\alpha)}{\alpha^2 M(\alpha)} \\
&\stackrel{log-sobolev}{\le} \frac{ C \int_{\R} e^{\alpha f(t)} \alpha^2 | \nabla f(t) | ^2 d \mu(t)}{\alpha^2 M(\alpha)}  = C \int_{\R} \frac{ e^{\alpha f(t)} }{M(\alpha)}  | \nabla f(t) | ^2 d \mu(t) 
\end{split}
\end{equation}
 
\item
\begin{equation}
\label{eq:lambda_zero}
\begin{split}
H(0) &= \frac{\log M(0)}{0} \stackrel{l'Hopital} = \frac{M'(0) / M(0) }{1} \\ &= \int_{\R} e^{0 f(t)} f(t) d\mu(t) / \int_{\R} e^{0 f(t)} d\mu(t)  =  \int_{\R} f(t) d\mu(t) = \E[f]
\end{split}
\end{equation}
\end{enumerate}


Now if we consider, 
\begin{equation}
\label{eq:h_int}
H(\lambda) - H(0) = \int_0^\lambda H'(\hat \alpha) d \hat \alpha \stackrel{\hat \alpha = \lambda \alpha}{=} \lambda \int_0^1 H'(\alpha) d\alpha
\end{equation}

Combining Eq.~\ref{eq:mgf} and Eq.~\ref{eq:h_int} we get,
\begin{equation}
\label{eq:lambda_e}
M(\lambda) = e^{\lambda H(\lambda)} = e^{\lambda H(0) + \lambda^2 \int_0^1 H'(\alpha) d\alpha } 
\end{equation}

\adios{This recursive definition always throws me off, can we give some intuition/better explaining it?}
 
Combining Eq.~\ref{eq:lambda_e}, Eq.~\ref{eq:lambda_derv}, and Eq.~\ref{eq:lambda_zero} and we get,
\begin{equation}
\label{eq:mgfb}
M(\lambda) \le e^{\lambda \E[f] + C \lambda^2 \int_{\R}  \int_0^1 \frac{ e^{\alpha f(t)} }{M(\alpha)}  | \nabla f(t) | ^2 d \mu(t) d \alpha } 
\end{equation}


Now, we can derive our new PAC-Bayesian bound for Bayesian Neural Networks. Starting from Theorem~\ref{thm:alquir}. Consider the following: 
\adios{better explain the conversion to expectation from average}

\begin{equation}
\label{eq:gs}
\begin{split}
\E_{w \sim p, S \sim D^m}  [ e^{ \lambda G_S(w) } ] &= \E_{w \sim p} \prod_{i=1}^m \E_{(x_i, y_i) \sim D} [ e^{ \frac{\lambda}{m} (\E_{z \sim D} \ell(w, x, y) - \ell(w, x_i, y_i))  } ] \\ &= \E_{w \sim p} e^{\lambda \E_{(x, y) \sim D} \ell(w, x, y)} \Big(\E_{(\hat{x}, \hat{y}) \sim D} [ e^{ \frac{\lambda}{m} (- \ell(w, \hat{x}, \hat{y}))  } ] \Big)^m 
\end{split}
\end{equation}

Notice, we can define $M(\alpha) = \E_{(x,y) \sim D} e^{\alpha f(w, x, y)}$. With combining Eq.~\ref{eq:mgfb} and Eq.~\ref{eq:gs}, we can derive the following, 
\begin{equation}
\label{eq:pac-bound-general-1}
\begin{split}
\E_{(x, y)  \sim D} [ e^{ \frac{\lambda}{m} (f(w,  x, y))} ] &\le \\ &e^{\frac{\lambda}{m} \E_{(x, y) \sim D}[f(w, x, y)] + C (\frac{\lambda}{m})^2 \E_{(x, y) \sim D}[ \| \nabla_{x} f(w, y, x) \| ^2 \int_0^1 \frac{ e^{\alpha  f(w, x, y)} }{M(\alpha)}  d \alpha] } \\
\Big(\E_{(x, y)  \sim D} [ e^{ \frac{\lambda}{m} (f(w, x, y))c }]\Big)^m &\le \\ &e^{\lambda \E_{(x, y) \sim D}[f(w, x, y)] + C \frac{\lambda^2}{m} \E_{(x, y) \sim D}[ \| \nabla_{x} f(w, x, y) \| ^2 \int_0^1 \frac{ e^{\alpha f(w, x, y)} }{M(\alpha)}  d \alpha] } \\
\end{split}
\end{equation}

Overall we get,
\begin{equation}
\label{eq:pac-bound-general-2}
\begin{split}
\E_{w \sim p, S \sim D^m}&  [ e^{ \lambda G_S(w) } ]  \\ \le~&\E_{w \sim p} e^{\lambda \E_{(x, y) \sim D} [f(w, x, y)]}  e^{\lambda \E_{(x, y) \sim D}[f(w, x, y)] + C \frac{\lambda^2}{m} \E_{(x, y) \sim D}[ \| \nabla_{x} f(w, ,x, y) \| ^2 \int_0^1 \frac{ e^{\alpha f(w, x, y)} }{M(\alpha)}  d \alpha] } \\
=~&\E_{w \sim p} e^{C \frac{\lambda^2}{m} \E_{(x, y) \sim D}\big [ \| \nabla_{x} f(w, x, y) \| ^2 \int_0^1 \frac{ e^{\alpha f(w, x, y)} }{M(\alpha)}  d \alpha \big] }
\end{split}
\end{equation}

\paragraph{Deep Neural Networks:}
We would like to stress here that the proposed bound can be directly applied to deep nets using different loss functions. In order to do so, one needs to compute the gradients w.r.t the input and plug it into Eq.~\ref{eq:pac-bound-general-2}.

%The complexity of learning the posterior $q$ is measured by the KL-divergence to the prior $p$. The KL-divergence between two $d$-dimensional Gaussian distributions: (1) the posterior distribution $q$ denoting the probability density of $N(\mu_q, \operatorname{diag}(\sigma_q^2))$; 
%(2) the prior distribution $p$ referring to the probability density of $N(0, \sigma_p^2 I)$ is analytically computable via
%\[
% \frac{1}{2} \left(d\log \sigma_p^2 - d -\! \sum_{i=1}^d \log \sigma^2_{q, i} + \frac{\|\sigma_q\|^2 + \|\mu_q\|^2}{\sigma_p^2} \right).\nonumber
%\]
%
%The above generalization gap $G_S(w) = L_D(w) - L_S(w)$ implies an optimization to the risk of the learner $L_D(w)$, as the generalization bound in Theorem \ref{theorem:t} takes the form $L_D(w) \le L_S(w) + C_1 KL(N(\mu_q, \operatorname{diag}(\sigma_q^2)) || N(0, \sigma_p^2 I)) + C_2$ for some $C_1, C_2$. 

%(1) due to instance normalization the NLL loss $\ell_\text{nll}(w,x,y)$ is bounded by a function of the weights of the top layer $B(W_k)$; (2) although the function $B(w)$ is unbounded, its average with respect to the variational dropout is small. 

%Our main theorem shows: (1) due to instance normalization the NLL loss $\ell_\text{nll}(w,x,y)$ is bounded by a function of the weights of the top layer $B(W_k)$; (2) although the function $B(w)$ is unbounded, its average with respect to the variational dropout is small. 

%We prove this when the variational dropout prior $N(0, \sigma_p^2 I)$ consists of $d$ independent Gaussian random variables, each with zero mean and the same variance $\sigma_p^2$. We also consider the variational dropout posterior distribution $N(\mu_q, \operatorname{diag}(\sigma_q^2))$, which consists of $d$ independent Gaussian random variables, each with a different mean $\mu_q = (\mu_{q,1},\ldots,\mu_{q,d})$ and variance $\sigma_q^2 = (\sigma^2_{q,1},\ldots,\sigma^2_{q,d})$.
%
%\begin{theorem}
%\label{theorem:t}
%Consider the generalization gap $G_S(w) = L_D(w) - L_S(w)$ of a $(k+1)$-layered deep net with parameters $w = (W_0,\ldots,W_k)$ which is trained with the NLL loss function $\ell_\text{nll}(w,x,y)$. Let $p$ be the probability density function of $N(0, \sigma_p^2 I)$ with variance $\sigma_p^2 \le 0.3$, which is the prior distribution over the parameters $w$.  With probability at least $1-\delta$ over the draw of the training set $S$  the following holds simultaneously for any posterior probability density function $q$ whose posterior distribution is $N(\mu_q, \operatorname{diag}(\sigma_q^2))$: 
%
%\[
%\E_{w \sim q} [G_S(w) ]  \le \frac{\frac{(\log c)^2}{4} + c\cdot d_k +  KL(q || p) + \log(1/\delta)}{\sqrt{m}} \nonumber 
%\]
%
%\end{theorem}  
%The proof consists of three steps which we outline first and detail in the supplementary material:
%\vspace{-\topsep}
%\begin{enumerate}\setlength{\parskip}{0pt}\setlength\itemsep{0pt plus 1pt}
%\item We use the notion of instance normalization to derive a weight dependent bound  $B(w) = \max_{x,y} \ell_{nll}(w,x,y)$ for the loss. We show that $B(w) \le 2 \|W_k\|_{\infty,2} + \log c$, where $c$ is the number of classes and $\|W_k\|_{\infty,2} = \max_y \|w_{k,y}\|_2$ is the matrix $L_{\infty,2}-$norm on the rows $w_{k,y}$ of the matrix $W_k$. 
%\item We apply the Hoeffding bound to the moment generating function $\E_{S \sim D^m}  [ e^{ \lambda G_S(w) } ] \le e^{\frac{\lambda^2 B(w)^2}{8m}}$ and set $\lambda = \sqrt{m}$. 
%\item We use the variational dropout prior to realize an average bound  $\log \E_{w \sim N(0,\sigma_p^2)}  [ e^{B(w)^2 } ] \le \frac{(\log c)^2}{4} + c\cdot d_k $. 
%\end{enumerate}
%A detailed description of the proof can be found in the supplementary material. The above bound depends on the number of parameters in the topmost layer $c\cdot d_k$. This can be reduced to $c^2$ by applying another layer on top of it with $c$ neurons. Such layers are typically used to learn an additional embedding of their input vector in the  $c$-dimensional decision space.

%The complexity of learning the posterior $q$ is measured by the KL-divergence to the prior $p$. The KL-divergence between two $d$-dimensional Gaussian distributions: (1) the posterior distribution $q$ denoting the probability density of $N(\mu_q, \operatorname{diag}(\sigma_q^2))$; 
%(2) the prior distribution $p$ referring to the probability density of $N(0, \sigma_p^2 I)$ is analytically computable via
%\[
% \frac{1}{2} \left(d\log \sigma_p^2 - d -\! \sum_{i=1}^d \log \sigma^2_{q, i} + \frac{\|\sigma_q\|^2 + \|\mu_q\|^2}{\sigma_p^2} \right).\nonumber
%\]
%
%The above generalization gap $G_S(w) = L_D(w) - L_S(w)$ implies an optimization to the risk of the learner $L_D(w)$, as the generalization bound in Theorem \ref{theorem:t} takes the form $L_D(w) \le L_S(w) + C_1 KL(N(\mu_q, \operatorname{diag}(\sigma_q^2)) || N(0, \sigma_p^2 I)) + C_2$ for some $C_1, C_2$. 
